Refined Commonsense Knowledge from Large-Scale Web Contents

Commonsense knowledge (CSK) about concepts and their properties is helpful for AI applications. Prior works, such as ConceptNet, have compiled large CSK collections. However, they are restricted in their expressiveness to subject-predicate-object (SPO) triples with simple concepts for S and strings for P and O. This paper presents a method called ASCENT++ to automatically build a large-scale knowledge base (KB) of CSK assertions, with refined expressiveness and both better precision and recall than prior works. ASCENT++ goes beyond SPO triples by capturing composite concepts with subgroups and aspects, and by refining assertions with semantic facets. The latter is essential to express the temporal and spatial validity of assertions and further qualifiers. Furthermore, ASCENT++ combines open information extraction (OpenIE) with judicious cleaning and ranking by typicality and saliency scores. For high coverage, our method taps into the large-scale crawl C4 with broad web contents. The evaluation with human judgments shows the superior quality of the ASCENT++ KB, and an extrinsic evaluation for QA-support tasks underlines the benefits of ASCENT++. A web interface, data, and code can be accessed at https://ascentpp.mpi-inf.mpg.de/.

==> Juliens_parts_backup/evaluation_mapping.tex <==
In Section~\ref{subsec:conceptnet_mapping}, we introduce methods to map our open knowledge base into a fixed-schema knowledge, ConceptNet here. Evaluating the mapping directly can be an unclear and challenging task. It does not consider that several OpenIE triples can generate the identical final triple, thus modifying the final ranking. So, we decided to evaluate the final generation instead.

Using a manual mapping of the relations, we generated a knowledge base containing 2 million statements. For the LM-based method, we generated the top ten ConceptNet triples for each statement, and we obtained a knowledge base containing ten million triples.

Besides the baselines introduced in Section~\ref{subsec:conceptnet_mapping}, we generated a knowledge base using only a language model. We used the model provided by COMET~\cite{comet-atomic-2020}. This model was finetuned to generate triples in ConceptNet. For each subject in our knowledge base and each predicate in ConceptNet, we generate ten candidates statements. They all come with a generation score that we use for an overall ranking. The resulting knowledge base contains 1.7 million triples.

To do so, we can build an automatic evaluation tool that compares our mapped knowledge base with our ideal target, ConceptNet. First, we compute the overlap between a mapped knowledge base and ConceptNet. The results are in Table~\ref{tab:overlap_conceptnet}.

\begin{table}[t]
    \centering
    \caption{Overlap between a generate knowledge base and ConceptNet. We indicate in the parenthesis the number of triples that were not present in the training dataset.}
    \begin{tabular}{|c|c|}
    \hline
        Method & Triples in ConceptNet \\
        \hline
        Manual Mapping & 1,589 \\
        LM-based Mapping & 12,901 (6,300) \\
        COMET (No Mapping) & 2,423 (763) \\
        \hline
    \end{tabular}
    
    \label{tab:overlap_conceptnet}
\end{table}

Next, we can compute Precision@k directly by comparing the top k elements in our new knowledge base with ConceptNet. Although it is not an accurate measurement, it still gives a lower bound that can be refined with manual annotations. The results are in Table~\ref{tab:precision_overlap}.

\begin{table}[t]
    \centering
        \caption{Precision@K for the overlapping with ConceptNet}
    \begin{tabular}{|c|c|c|c|c|}
    \hline
        Method & P@10 & P@100 & P@1000 & P@10000 \\
        \hline
        Manual Mapping & 0.0\% & 4\% & 4\% & 1.74\% \\
        LM-based Mapping & \textbf{90\%} & \textbf{62\%} & \textbf{30.4\%} & \textbf{10.2\%} \\
        COMET (No Mapping) & 20\% & 12\% & 5\% & 1.13\% \\
        \hline
    \end{tabular}
    \label{tab:precision_overlap}
\end{table}

==> Juliens_parts_backup/lm_based_mapping.tex <==
\subsubsection{LM-boosted mapping}

Builds on LM-based seq-to-seq model. It has three unique traits:
\begin{enumerate}
    \item Can turn one open assertion into several closed ones
    \item Can invert relations
    \item Can modify object and subject.
\end{enumerate}
These added freedoms allow to correct extractions and to get stronger frequency signals. But, at the same time, they imply that the close link to the extraction source sentences may get lost.



To perform an LM-model-based mapping, we proceed in two steps. The first one consists in creating a dataset of alignments. This process could be done manually to obtain high-quality data. However, that would require a lot of qualified human labor, be expensive to run, and not generalize to other knowledge bases. Therefore, we decided to adopt an automatic alignment algorithm. Given an OpenIE triple, we want to find, if possible, the most likely translation in ConceptNet. Even if the translation is not perfect, we hope the more considerable amount of training data will help the system generalize.

The algorithm we use simply tackle the problems we might encounter when aligning an OpenKB with a fixed-schema KB (here, we consider ConceptNet). We works as follows:

\begin{enumerate}
    \item We lemmatize the predicates (if possible) and the objects from the OpenKB and ConceptNet and remove stopwords.
    \item For each triple $(s, p, o)$ in our OpenKB, we create one or several alignments if (we used \_ as a general placeholder):
    \begin{itemize}
        \item s, \_, o is in Conceptnet (standard alignment)
        \item o, \_, s is in Conceptnet (reverse alignement)
        \item s, \_, p + o is in Conceptnet (predicate in the object)
        \item p + o, \_, s is in Conceptnet (reverse predicate in the object)
    \end{itemize}
\end{enumerate}


Then, the second step consists in finetuning a language model to generate the alignments. In our experiments, we used the GPT2 model~\cite{radford2019language} and the script provided by HuggingFace to train GPT2. Finally, we formatted our input by separating the OpenIE triple and its aligned ConceptNet triple with a \textit{[SEP]} token.

We used a beam search for the generation part to obtain the top K results for each statement in our knowledge base. Considering more than one alignment per triple can help in many ways. First, a triple can have several translations. Second, we observed that the system learned to generate related statements that might help when ranking the final statements.

Once we have all the translations to ConceptNet triples, we compute a score for each triple based on the frequency at which it appeared (several OpenIE triples generally generate the same ConceptNet triple) and the inverse rank among the prediction. For formally, the score of a triple $t$ is computed using:

\begin{align*}
score(t) = \sum_{\text{t' generates t}} \frac{score(t')}{rank(t', t) + 1}
\end{align*}

In the end, we are able to generate a ranking of all our statements.

==> Juliens_parts_backup/motivation_mapping.tex <==
\subsubsection{Motivation And Challenges}

We provide an open knowledge base, with no constraint on the predicates. However, some people might prefer to use a knowledge base with a fixed-schema like ConceptNet. The fixed-schema knowledge bases are more popular, and therefore more applications (like question-answering or entity-linking) are developed for them. This is particularly the case for commonsense, there ConceptNet is by far the most used knowledge base.

By reducing the number of predicate, we will also be able to increase the quality of a knowledge base as several open triples might generate the same final triple. For example, \textit{fish, live in, water}, \textit{fish, swim in, water} and \textit{fish, breath in, water} can be aligned to \textit{fish, LocatedIn, water} in ConceptNet, and therefore help to consolidate that statement.

Mapping open triples to a fixed-schema raises many challenges that come from the fact that align an OpenKB with a fixed-schema KB is not trivial. In the easiest case, the subject and the object are the same in both KBs, and we just have to predict the correct predefined predicate. This would be a classification task. For example, \textit{fish, live in, water} can be mapped to \textit{fish, LocatedAt, water} in ConceptNet. We could proceed similarly in the case where the subject and the object are inverted, like in \textit{ocean, contain, fish} that can be mapped to \textit{fish, LocatedAt, ocean}. Therefore, we should also consider inverse relations. In some cases, the object is not expressed in the same way, or only partially: \textit{fish, live in, the ocean} can be mapped to \textit{fish, LocatedAt, ocean}. In other cases, part or all of the predicate is in the object, like in \textit{fish, swim in, the ocean} that can be mapped to \textit{fish, CapableOf, swim in the ocean}. Here also, the initial triple could also be mapped to \textit{fish, LocatedAt, ocean}, showing that the mapping is not always unique. Other problems might also arise, like the alignment of synonyms.

==> parts/biographies.tex <==
% author biographies
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/phong}}]{Tuan-Phong Nguyen}
is
a Ph.D. candidate in Department of Databases and Information Systems at the Max Planck Institue for Informatics and the International Max Planck Research School on Trustworthy Computing. His research interests span Commonsense Knowledge Base Construction, Information Extraction and Natural Language Processing.
Previously, he obtained his MSc. degree from Saarland University (2020) and BSc. degree from Vietnam National University Hanoi (2016), both in Computer Science.
\end{IEEEbiography}

% author biographies
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/simonrazniewski}}]{Simon Razniewski}
is senior researcher at the Max Planck Institute for Informatics in Saarbrücken, Germany, where he heads the Knowledge Base Construction and Quality area.
He was previously assistant professor at the Free University of Bozen Bolzano (2014-2017). He holds a PhD from the Free University of Bozen-Bolzano (2014), and a Diplom (MSc.) from TU Dresden (2010). He spent time as visitor at the Max-Planck Institute for Informatics (2016), the University of Queensland (2015), AT\&T Labs-Research (2013), the University of California, San Diego (2012), and has previous industrial experience from Globalfoundries (2010) and Siemens IT (2009).
\end{IEEEbiography}

% author biographies
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/julienromero.jpg}}]{Julien Romero} is an associate professor at Telecom SudParis, France, in the SAMOVAR lab. Before that, he made a postdoc at the Max Planck Institute of Informatics. (2020-2021) He obtained a Ph.D. in computer science from Telecom Paris, France, in 2020, a master of science from the ETH, Zürich, Switzerland, and an engineering diploma from Telecom Paris. His research interests cover knowledge bases, information extraction, natural language processing, and databases.
\end{IEEEbiography}

% author biographies
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/gerhardweikum}}]{Gerhard Weikum}
is a Scientific Director at the Max Planck Institute for Informatics in Saarbruecken, Germany, and an Adjunct Professor at Saarland University. He co-authored a comprehensive textbook on transactional systems, received the VLDB Test of Time Award for his work on automatic database tuning, and is one of the creators of the YAGO knowledge base which received the WWW Test of Time Award. 
%He has served on the editorial boards of ACM TODS, IEEE TKDE and ACM TWEB, and was PC chair of ACM SIGMOD and IEEE ICDE. 
%Among various honors, 
He is an ACM Fellow and received the ACM SIGMOD Edgar F. Codd Innovations Award.
\end{IEEEbiography}


==> parts/model_architecture.tex <==
\section{Model and Architecture}

\subsection{Knowledge model}
\label{subsec:model}

Existing CSKBs typically follow a triple-based data model, where subjects are linked via predicate phrases to object words or phrases. Typical examples, from ConceptNet, are \triple{bus, UsedFor, travel} and \triple{bus, UsedFor, not taking the subway}.

Few projects~\cite{webchild,mishra2017domain} have attempted to sharpen such assertions by word sense disambiguation (WSD) \cite{DBLP:journals/csur/Navigli09}, distinguishing, for example, buses on the road from computer buses.
Likewise, only a few projects~\cite{DBLP:conf/aaaifs/GordonS10,zhang2017ordinal,quasimodo,chalier2020joint}, have tried to identify salient assertions against correct ones that are unspecific, atypical, or even misleading (e.g., buses used for avoiding the subway or used for enjoying the scenery).
We extend this prevalent paradigm in two significant ways.

\paragraph{Expressive subjects} 
%\GW{this is a little long and repeats some of the intro's points - needs trimming}\\
%Standard problems in knowledge representation are to define what is considered as entity, and how to decide whether two entities are the same or not. Knowledge bases like ConceptNet do not disambiguate lexical surface terms, leading to odd effects like shown in Fig.~\ref{fig:kr-subjects}, where elephant trunks become locations of spare tires.
CSK acquisition starts by collecting assertions for target subjects, which are usually single nouns. This has two handicaps: 1) it conflates different meanings for the same word, and 2) it misses out on refinements and variants of word senses. While some projects~\cite{webchild,mishra2017domain} tried to use word sense disambiguation (WSD) to overcome the first issue, they were inherently limited by the underlying word-sense lexicons (WordNet or Wiktionary). Indeed, they mainly restrict themselves to single nouns. For example, phrases like ``city bus'' or ``tourist bus'' are not present. 

%A step forward is to use sense disambiguation, popularly to WordNet~\cite{wordnet}, such that car trunks and animal trunks become separate concepts. This approach is taken, for instance, by TupleKB. Traditional word sense disambiguation, however, does not solve a more subtle problem: Elephant trunks and anteater trunks are quite different in size, purpose, and even anatomic origin, so assertions like \term{trunks are used for carrying branches}, applicable for elephants, are incorrect for anteaters. Limited sets of word senses (e.g., WordNet knows just 5 senses each for the terms trunk, ear, and tooth), cannot capture this. 
%\GW{this gives very high importance to WSD -- but then, we don't do this either! I would rather say that WSD is not a solution because multi-word phrases are crucial and hardly covered by sense lexicons like WordNet or Wiktionary!!!}\\
%\GW{the anteater trunk is even more tricky: this is not just an issue of capturing important multi-word phrases, but it could open up Pandora's box of having to understand full context -- for example, on could argue: what about SUV trunk, mini trunk, cargo trunk, etc. etc. -- and we don't address this really!}

%\begin{figure}
%    \centering
%    \includegraphics[width=.35\textwidth]{figures/kr-subjects.pdf}
%    \caption{Issues arising from lack of word sense disambiguation in ConceptNet.}
%    \label{fig:kr-subjects}
%\end{figure}

Our approach to rectify this problem is twofold:
\squishlist
    % \item First, our source discovery method combines the target subject with an informative hypernym (using WordNet, applied to single nouns or head words in phrases). For example, instead of searching with the semantically overloaded word ``bus'', we generate queries ``bus public transport'' and ``bus network topology'' to disentangle the different senses. \jr{This was the case for Ascent, but not for Ascent++, wasn't it?}
    
    \item \newmaterial First, when discovering source documents for the target subject, we compare the documents with its reference Wikipedia article, and then only retain documents with better similarity. This way, we can disentangle different senses, for example, of ``bus'' as in ``public transport'' and ``network topology'' themes.
    
    \item \oldmaterial Second, when extracting candidates for assertions from the source documents,
    % retrieved web pages, 
    we capture also multi-word phrases as candidates for refined subjects, such as ``school bus'', ``city bus'', ``tourist bus'', ``circus elephant'', ``elephant cow'', ``domesticated elephant'', etc. This way, we can acquire {\em isa}-like refinements, to create {\em subgroups} of broader subjects, and also other kinds of {\em aspects} that are relevant to the general concept. An example for the latter would be ``bus driver'' or, for the target subject ``elephant'', phrases such as ``elephant tusk'', ``elephant habitat'' or ``elephant keeper''.
\squishend

%We therefore propose to keep each salient part or \textit{aspect} of a subject as separate concepts, each collecting their own assertions. Unlike haspartKB \cite{???}, our goal is not to collect an exhaustive, nested collection of meronymy, but instead, to collect salient parts and aspects that come with own assertions. We therefore also do not limit the scope to physical parts (trunk, ears, legs), but allow any salient aspects such as habitat, diet, cognition.
%\GW{this talks about *aspects* -- is this the same as *facets* ? if not, it needs to made much clearer that *aspects* refine subjects (but later the terminology is sub-groups, is this the same as aspects ?) and that *facets* refine the entire assertions (or the PO components) !?}

%Beyond aspects of subjects, we also include \textit{subgroups} \GW{what is the diff betwee aspects and sub-groups?}, 
%transcending 
Our notion of {\em subgroups} can be thought of as an inverse {\em isa} relation. It goes beyond traditional taxonomies by better coverage of multi-word composites (e.g., ``circus elephant''). This allows us to improve the representation of specialized assertions such as \triple{circus elephants, catch, balls}.

Our notion of {\em aspects} includes part-whole relations (PartOf, MemberOf, SubstanceOf)~\cite{DBLP:journals/coling/GirjuBM06,shwartz2018olive,tandon2016commonsense,haspartkb}, but also further aspects that do not fall under the themes of hypernymy or meronymy. Examples are ``elephant habitat'' or
``bus accident''. Note that, unlike single nouns, such compound phrases are rarely ambiguous, so we have crisp concepts without the need for explicit WSD.
%extending
%traditional taxonomies (African and Asian elephant), and incorporating activity- and property-based subgroups such as baby elephants, foraging elephants, and work elephants (for attempts at further classifying these see e.g., \cite{shwartz2018olive,tandon2016commonsense,haspartkb}). Incorporating these subjects allows us a much finer-grained modelling of commonsense, as for instance, only male lions have manes, and only circus elephants play tricks.

\paragraph{Semantic facets} For CSK, assertion validity often depends on specific temporal and spatial circumstances, e.g., elephants scare away lions only in Africa or bathe in rivers only during daytime. 
Furthermore, assertions often become crisper by contextualization in terms of causes/effects and instruments (e.g., children ride the bus \dots to go to school, circus elephants catch balls \dots with their trunks).

%or transitive objects of verbs like ``give'' and ``take''.


% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.65\textwidth]{figures/elephant-data-model.pdf}
%     \caption{Example of \ascentpp's knowledge for the concept \emph{elephant}. The data model of traditional CSKBs like ConceptNet is restricted to assertions outside the green box.}
%     \label{fig:examples}
% \end{figure*}


To incorporate such information into an expressive model, we choose to contextualize subject-predicate-object triples with semantic {\em facets}. To this end, we build on ideas from research on semantic role labeling (SRL)~\cite{DBLP:series/synthesis/2010Palmer,clarke2012nlp,semanticrolelabelling}.
%\GW{very good point here, some of this must also be said in Related Work, with SRL references}
This line of research has been initially devised to fill hand-crafted frames (e.g., purchase) with values for frame-specific roles (e.g., buyer, goods, price, etc.).
We start with a set of 35 labels proposed in~\cite{stuffie}, a combination of those in the Illinois Curator SRL~\cite{clarke2012nlp}, and 22 hand-crafted ones derived from an analysis of semantic roles of prepositions in Wiktionary.
As many of these are very special, we condense them into eight widely useful roles that are of relevance for CSK: four that qualify the validity of assertions (\textit{degree}, \textit{location}, \textit{temporal}, \textit{other-quality}), and four that capture other dimensions of context (\textit{cause}, \textit{manner}, \textit{purpose}, \textit{transitive objects}).

These design considerations lead us to the following knowledge model.
%Fig.~\ref{fig:examples} shows an example with several CSK assertions.

%\paragraph{Model}
%\begin{definition}[Commonsense Assertion] 
%%%GW: this is the only def in the paper, no need for numbering and special latex env
\vspace*{0.2cm}
\noindent{\bf Definition [Commonsense Assertion]:}\\
Let $C_0$ be a set of primary concepts of interest, which could be manually defined or taken from a dictionary. \\
Subjects for assertions include all $s_0 \in C_0$ as well as judiciously selected
multi-word phrases that contain some $s_0$.\\
Subjects are interrelated by {\em subgroup} and {\em aspect} relations: each $s_0$ can be refined by a set of subgroup subjects denoted $sg({s_0})$, and by a set of aspect subjects denoted $asp({s_0})$. The overall set of subjects is $C := C_0 \cup sg_{C_0} \cup asp_{C_0}$.\\


A commonsense assertion for $s \in C$ is a quadruple \triple{s, p, o, F} with single-noun or noun-phrase subject $s$, short phrases for predicate $p$ and object $o$ and a set $F$ of semantic facets.
Each facet $(k,v) \in F$ is a key-value pair with one of eight possible keys $k$ and a short phrase as $v$.
%GW: a set of key-value pairs denoting semantic facets,
%where the keys are among the eight types listed above, and the values are short text phrases.
%Note that each assertion can have multiple facets, though only one per facet key. \sr{The following is not true: ``
Note that a single assertion can have multiple key-value pairs with the same key (e.g., different spatial phrases).
%'' - as this doesn't make sense for degree, for example, we consolidate facet values per facet type into a single value. Though I see that that has shortcomings too - something to revisit in extensions!} \ph{Actually we currently allow more than one values per facet type. I think except for degree, all other face types can store multiple facet values (see e.g. Fig. 1, <elephant sucks water> has 2 purposes.)}
\hspace*{0pt}\hfill $\qed$
%\end{definition}
% \vspace*{0.1cm}

%\GW{needs to explain $sg...$ and $asp...$
%and clarify aspects vs. subgroups vs. facets;
%also, I would refer to facets as key-value pairs rather than a map, but this is a minor point}\\
%\GW{the example figure with the elephants should be re-drawn so that all S's are aligned, all P's are aligned, all O's are aligned and all F's are aligned -- in the current form it is easy to misinterpret elephant ear is an object ...!}\\
%\GW{also the figure does not help to clarify aspects vs. subgroups! and couldn't one argue that what is shown as one quadruple here could be easily split into several simpler tuples, say
%1) elephant hasSubPart elephant tusk, and
%2) elephant tusk contains 40000 muscles???
%in other words: why is hasSubPart treated differently from other predicates??? is this an artificial consequence from the collection procedure that starts with single-noun subjects? or is there a semantic principle here? if so, it does not come across}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%Our goal is to extract \triple{subject, predicate, object} triples, enhanced with qualitative (textual) facets that either render more precise the validity of an assertion. 

%We also noticed that salient assertions about a concept often concern subsets, or subparts of a concept. For instance, a salient assertion for \ex{lynx tails have a black tip}, or that \ex{female lynx are sole caretakers}. These do not fit into triples with \ex{lynx} as subject, yet are not assertions about tails or females in general either, so we introduce two special predicates, \ex{hasSubGroup} and \ex{hasSubPart}, which allow us to tightly couple these assertions with the generic subject. Although a few existing works have collected subgroups (e.g., ConceptNet knows 11 subtypes of pilots) or parts (WebChild, hasPartKB \cite{haspartkb}), none of them collects assertions for subgroups and subparts.

%In this work we adopt a pragmatic definition of subgroups and subparts. For the subgroups we allow both instance-based subgroups (e.g., \ex{African elephant}, \ex{male elephant}), as well as state- and activity-based subgroups (e.g., \ex{foraging elephant}, \ex{old elephant}). For subparts we both consider physical parts (tusks of an elephant, robe of a lawyer), as well as conceptual parts of their domain (e.g., life of an elephant, client of a lawyer). Further classifications have been attempted (see e.g., \cite{shwartz2018olive,tandon2016commonsense,haspartkb}, but all have limitations, and so we do not organize subparts and subgroups further, but rely on frequency for identifying salient ones.



%In summary, our output for a given subject $s_0$ consists of:
%\begin{enumerate}
%    \item Assertions $(s,p,o,\mathcal{F})$ of open predicates and objects, along with optional semantic facets $\mathcal{F}=\{f_1,\dots,f_8\}$ where $f_i$ demonstrates \textit{location, temporal, degree, other-quality, cause, manner, purpose, transitive object};
%    \item Assertions $(s,\textit{hasSubPart},o)$ of salient subparts of $s_0$;
%    \item Assertions $(s,\textit{hasSubGroup},o)$ of salient subgroups of $s_0$;
%    \item Assertions $(s',p,o,\mathcal{F})$, where $s'$ is a subpart or subgroup of $s_0$.
%\end{enumerate}
% An example of assertions for $s_0=\text{elephant}$ is shown in Fig.~\ref{fig:examples}.

\newmaterial

%\ascentpp{} inherits the same knowledge model from \ascent{}. Moreover, because of the high-quality extraction of subgroups and aspects already conducted in \ascent{} (cf. Section 5.2 in~\cite{ascent}), we simply transfer the top subgroups and aspects in \ascent{} to \ascentpp{} and eliminate the component of fine-grained term extraction.

\oldmaterial


\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/ascentpp.pdf}
    \caption{Architecture of the \ascentpp{} system.
    % \ph{TODO: Add example of outputs below each step.}
    }
    \label{fig:architecture}
\end{figure*}


\subsection{Extraction architecture}

\paragraph{Design considerations}
CSK collection has three major design points: (i) the choice of sources, (ii) the choice of the extraction techniques, and (iii) the choice of cleaning or consolidating the extracting candidate assertions.

As \textit{sources}, most prior works carefully selected high-quality input sources, including book n-grams~\cite{webchild}, concept definitions in encyclopedic sources, and school text corpora about science~\cite{clark2018think}. These are often a limiting factor in the KB coverage. Moreover, even seemingly clean texts like book n-grams come with a surprisingly high level of noise and bias (cf.~\cite{DBLP:conf/cikm/GordonD13}).
Focused queries for retrieving relevant web pages were used by~\cite{mishra2017domain}, but the query formulations required non-negligible effort. Query auto-completion and question-answering forums were tapped by Quasimodo~\cite{quasimodo}. While this gave access to highly salient assertions, it was, at the same time,
adversely affected by heavily biased and sensational contents (e.g., search-engine auto-completion for ``snakes eat'' suggesting ``\dots themselves'' and ``\dots children'').

%give access to highly salient knowledge, but come with considerable noise and skew. Web search engines are well suited to identify relevant documents, however, require query engineering, and can be costly~\cite{mishra2017domain}. 
% In \ascentpp{} we opt for using search engines for wide coverage, and devise
% techniques for quality assurance.
%as these are most promising for obtaining high-quality input in open domains.
\newmaterial
Search engines were also used in \ascent{}~\cite{ascent} in combination with refined search queries that use hypernyms for disambiguation. Then, each retrieved web page was compared with a reference document of its corresponding subject to make sure that the web page was not off-topic. This helped \ascent{} to collect very high-quality documents for various subjects such as animals (e.g., there are lots of web pages exclusively talking about animal facts). However, the method did not work well on subjects for which named instances are generally more prominent than the general concepts, such as ``university'' or ``car''. For instance, while for ``elephant'', the method extracted  508 assertions of frequency greater than one, for ``university'' it found a mere 12.
%That resulted in very sparse distribution of assertions for those subjects, for example, $97.9\%$ of $547$ assertions for ``university'' in \ascent{} have a frequency of $1$ after clustering. 
%Other subjects in the occupation and engineering domain did not reach the same coverage as the animal subjects either. By limiting to a few hundred of retrieval results, we missed out lots of other available sources.
\ascentpp{} rectifies this by directly using a huge corpus as extraction source. This approach was also taken by ASER~\cite{zhang2020aser} and its derivative, TransOMCS~\cite{DBLP:conf/ijcai/ZhangKSR20}, yet these approaches are recall-oriented and lack appropriate consolidation. 

\oldmaterial
For the \textit{extraction techniques}, choices range from co-occurrence- and pattern-based methods (e.g.,~\cite{elazar2019large}) and open information extraction (e.g.,~\cite{mishra2017domain,quasimodo}) to supervised learning for classification and sequence tagging. Co-occurrence works well for a few pre-specified, clearly distinguished predicates using distant seeds. Supervised extractors require training data for each predicate and thus have the same limitation. Recent approaches, therefore, prefer OpenIE techniques, and our
extractors follow this trend, too.
% \ascentpp{} reuses these extractors from \ascent{}.

For \textit{knowledge consolidation}, early approaches kept all assertions from the ingest process (e.g., crowdsourcing~\cite{conceptnet}), whereas recent projects employed supervised classifiers or rankers for cleaning~\cite{mishra2017domain,quasimodo,chalier2020joint,zhang2017ordinal}, and also limited forms of clustering~\cite{mishra2017domain,quasimodo} for canonicalization (taming semantic redundancy).
%Given our richer contextualization ranking by truth is not an issue in our resource, and given the careful choice of extraction sources, we find that extraction frequencies are generally a strong indicator of salient assertions.
% In \ourkb{}, the careful source selection already eliminates certain kinds of noise, rendering extraction frequency statistics a much better signal than in earlier works.
%Thus, instead of supervised reranking, our consolidation phase focuses on reinforcing frequency signals by assertion clustering, as redundancy is a pressing issue for open extraction schemes, using state-of-the-art pretrained language models.
% Therefore, we focus on reinforcing these signals for consolidation,
% based on clustering with contextual language models for informative similarity measures.
\newmaterial
In \ascent{}, we used contextual language models to cluster assertions of the same meanings and reinforce the frequency signals of those assertions. 
In the present \ascentpp{}, we apply the same technique with a state-of-the-art model for sentence embeddings which is the SentenceTransformers model~\cite{sbert}. Furthermore, after clustering, we do a mapping from our open-schema CSKB to the well-established ConceptNet schema as it is favorable to many researchers (e.g.,~\cite{comet-atomic-2020,lin2019kagnet,feng2020scalable}). Finally, a heuristic-based cleaning approach is applied to eliminate other remaining noise in the resulting KB.



% \vspace*{0.2cm}
\paragraph{Approach}
The new \ascentpp{} methodology operates in two phases (illustrated in Figure~\ref{fig:architecture}):
\squishlist
    \item[1.] \textit{Corpus processing}
    \squishlist
        \item[1a.] \textit{NLP pipeline}: Running NLP pipeline for the input corpus to get NLP features of all sentences, in particular part-of-speech tags and dependency trees.
        \item[1b.] \textit{Faceted OpenIE}: Running the \ascent{} OpenIE system to get faceted assertions from the processed sentences.
    \squishend
    \item[2.] \textit{Aggregation and consolidation}: in this phase, each subject is processed separately.
    \squishlist
        \item[2a.] \textit{Filtering}: Performing a series of document and assertion filtering to get relevant and high-quality assertions for a given subject.
        \item[2b.] \textit{Clustering} of retained assertions based on sentence embeddings.
        \item[2c.] \textit{Mapping} from open assertions into ConceptNet schema.
        \item[2d.] \textit{Cleaning} based on heuristics and a dictionary of unwanted assertions.
        \item[2e.] \textit{Ranking} of assertions: Annotating assertions with complementary scores for typicality and saliency.
    \squishend
\squishend
Both phases treat each document or subject independently, thus can be highly parallelized (see also Section~\ref{sec:implementation}).
% %\begin{enumerate}
% \squishlist
% %    \item Document retrieval;
% \item[1.] Source discovery:
% %    \begin{enumerate}
%     \squishlist
%         \item[1a.] Retrieval of web 
%         pages from search engines with specifically generated queries;
%         \item[1b.] Filtering of result pages based on similarity to Wikipedia reference articles.
%         \squishend
% %    \end{enumerate}
%     \item[2.] Extraction of assertions with subgroups, aspects and facets:
% %    \begin{enumerate}
%     \squishlist
%         \item[2a.] OpenIE for rule-based extraction using dependency-parsing patterns;
%         \item[2b.] Labeling of semantic facets by supervised classifier.
%     \squishend
% %    \end{enumerate}
%     \item[3.] Clustering of assertions based on contextualized embeddings.
% \squishend
% %\end{enumerate}
%
%\GW{these are 5 steps, but the intro said that ASCENT would be based on 3 phases -- this is confusing to the reader, need to restructure the 5 here into 3, e.g., by referring to 1a and 1b as sub-steps of source discovery, and so on!
%the preceding text clearly suggest 3 phases, too: 3 paragraphs on sources, extraction and consolidation!}\\
In the following, we discuss Phase 1, and each of the subphases 2a-2e in a separate subsection.






% \sr{New part starts here}

% Needs careful rethinking! How to arrange modules?

% Subject-centric, or OpenIE on whole corpus first, then group results by subject? 

% WordNet lemmas perhaps play no role anymore - we just go by surface terms?

% Coreference still needed for aspects?

% Re-ranking module needs thought - if we employ LMs, does that hurt our message? Probably not.

% The filtering of pages by containing several statements is sensible and can perhaps be expanded - this strongly suggests a subject-centric view (i.e., start with elephant, go over corpus of websites/extractions, and retain only a subset of all of them)




% \section{Methodology}

% \subsection{Relevant Document Retrieval}
% \label{subsec:docretrieval}

% \paragraph{Web search} 
% %Previous works have spent considerable effort on source selection, either manually selecting meta-resources (WebChild, Quasimodo), or judiciously designing specific search queries over the general web (TupleKB). In this work we adopt the idea of using the general web of TupleKB, but propose a generic and simple principle for removing irrelevant and/or noisy search results.
% We use targeted web search to obtain documents specific to each subject, this way aiming to reduce the noise from out-of-context concept mentions, and the processing of large collections of mostly irrelevant documents, like encountered for instance in general web crawls. This is especially relevant as we later utilize coreference resolution, which is by itself a source of additional noise. Specifically, we utilize the Bing Web Search API.%\footnote{\href{https://azure.microsoft.com/en-us/services/cognitive-services/bing-web-search-api/}{https://azure.microsoft.com/en-us/services/cognitive-services/bing-web-search-api/}}

% Given a concept $s_0$, we first map it to a corresponding WordNet synset by taking the synset with the most lemma names, and use its hypernyms to refine search queries. For example, if $s_0$ has hypernym \textit{animal.n.01} then its search query is ``$s_0$ animal facts'', or if $s_0$ has hypernym \textit{professional.n.01} then its search query is ``$s_0$ job descriptions'', etc. We have manually designed templates for 35 commonly encountered hypernyms.
% These cover 82.5\% of our subjects.
% % \sr{State coverage: ``These cover XYZ\% of our subjects''}
% When none of the templates can be applied, we default to the direct hypernym of $s_0$ and form the following search query: ``$s_0$ (hypernym)''. Below we provide an example of search query for the animal lynx whose WordNet synset is \textit{lynx.n.02}, and a few top results returned by Bing.

% \begin{quote}
%     \texttt{\small \textbf{Query:} lynx animal facts \\
%     \textbf{Top 5 results:}
%     \begin{itemize}
%         \item Lynx $\vert$ National Geographic
%         \item Interesting facts about lynx $\vert$ Just Fun Facts
%         \item Lynx Facts $\vert$ Softschools.com
%         \item Facts About Bobcats \& Other Lynx $\vert$ Live Science
%         \item Lynx $\vert$ Wikipedia
%     \end{itemize}}
% \end{quote}


% \paragraph{Document filtering} Commercial search engines give us the benefit that (near-)duplicates, e.g., copies from Wikipedia, are well detected and ranked lower. At the same time, the search engine goal of diversification may introduce spurious results, despite our efforts with the search query refinement. This is exacerbated by our interest to obtain large sets of articles. We therefore propose a filter to remove irrelevant results. Given a subject $s_0$, we use the Bing API to retrieve 500 websites. For each website, we use a popular article scraping library\footnote{\href{https://github.com/codelucas/newspaper}{https://github.com/codelucas/newspaper}} to scrape its main content. Next, each retrieved document is compared with a Wikipedia reference article by the cosine similarity of the bag of words of both pages. 
% As Wikipedia reference, we leverage the WordNet-Wikipedia pairings of BabelNet~\cite{navigli2012babelnet} and the resource by \cite{fernando2012mapping} as the first fallback. If both resources do not contain the desired WordNet synset, we simply pick the first Wikipedia article appearing in the search result.
% After this, only documents with similarity higher than 0.55 (chosen based on tuning on withheld data) are retained.
% % \GW{I guess document means full content of a web page, right? is there any kind of pre-processing here (boilerplate removal, more attention to page title, headings, links etc. ?)?}
% % \sr{I remember there was none - but say which framework used - BeautifulSoup/Scrapy?}
% % \ph{I added the framework reference.}


% \subsection{Knowledge Extraction}
% \begin{table*}[t]
% \centering
% \tiny
% \begin{tabular}{llll}
% \toprule
% \textbf{No.} & \textbf{Sentence} & \textbf{StuffIE~\cite{stuffie}} & \textbf{\ourkb{} OpenIE extractor} \\
% \midrule
% 1 & They eat ptarmigans, voles, and grouse. & (1) They; eat; ptarmigans, voles, and grouse & \begin{tabular}[c]{@{}l@{}}(1) They; eat; ptarmigans\\ (2) They; eat; voles\\ (3) They; eat; grouse\end{tabular} \\
% \midrule
% 2 & Lynx are active during evening and early morning. & \begin{tabular}[c]{@{}l@{}}(1) Lynx; are; active\\ (1.1) TEMPORAL: during evening and early morning\end{tabular} & \begin{tabular}[c]{@{}l@{}}(1) Lynx; are; active\\ (1.1) TEMPORAL: during evening\\ (1.2) TEMPORAL: during early morning\end{tabular} \\
% \midrule
% 3 & Lions live for 20 years in captivity. & \begin{tabular}[c]{@{}l@{}}(1) Lions; live; \_\\ (1.1) PURPOSE: for 20 years\\ (1.2) LOCATION: in captivity\end{tabular} & \begin{tabular}[c]{@{}l@{}}(1) Lions; live; for 20 years\\ (1.1) LOCATION: in captivity\end{tabular} \\
% \midrule
% 4 & Lions hunt many animals, such as gnus and antelopes. & (1) Lions; hunt; many animals, such as gnus and antelopes. & \begin{tabular}[c]{@{}l@{}}(1) Lions; hunt; gnus\\ (2) Lions; hunt; antelopes\end{tabular} \\
% \midrule
% 5 & Dogs are extremely smart. & (1) Dogs; are; extremely smart & \begin{tabular}[c]{@{}l@{}}(1) Dogs; are; smart\\ (1.1) DEGREE: extremely\end{tabular} \\
% \midrule
% 6 & Elephants are extremely good swimmers. & (1) Elephants; are; extremely good swimmers & \begin{tabular}[c]{@{}l@{}}(1) Elephants; are; good swimmers\\ (1.1) DEGREE: extremely\end{tabular}                                 \\
% \bottomrule
% \end{tabular}
% \caption{Comparison of outputs returned by our OpenIE method and StuffIE.}
% \label{tab:openie-examples}
% \end{table*}

% To enable the extraction of diverse pieces of information, our extraction step relies on open information extraction~\cite{DBLP:conf/ijcai/Mausam16,niklaus2018survey}. Similarly, as open assertions typically follow a general grammatical structure, we utilize dependency-path-based rules to identify extractions. We also rely on rules to identify aspects via possessive constructions, and subgroups via compound nouns. For assigning facets to semantic groups, we use supervised models, as the set of facets is small.



% \paragraph{Rule-based statement extraction} Our open information extraction (OpenIE) method builts upon the StuffIE approach~\cite{stuffie}, a series of hand-crafted dependency-parse-based rules to extract triples and facets. The core ideas are to consider each verb as a candidate predicate of an assertion, and to identify subjects, objects and facets via grammatical relations, so-called dependency paths. The elaboration below uses the Clear style format (\url{http://www.clearnlp.com}), as used by the spaCy dependency parser:
% \begin{itemize}
%     \item Subjects are captured based on dependencies of the type subject (\code{nsubj}, \code{nsubjpass} and \code{csubj}) and  adjectival clauses (\code{acl}). If no subject is found, the parent verb of the predicate identified through adverbial clause modifier (\code{advcl}) and open clausal complement (\code{xcomp}) edges is used to identify subjects.
%     \item Dependency edges used to find objects are direct object (\code{dobj}), indirect object (\code{iobj}), nominal modifier (\code{nmod}), clausal complement (\code{ccomp}) and adverbial clause modifier (\code{advcl}). % whereas using the latter two results in nested relations because the extracted object is a verb (i.e., predicate of another triple).
%     \item Once a triple has been formed, its constituents are completed by expanding their head words with related words via various dependency edges. For compound predicates, these include \code{xcomp}, \code{auxpass}, \code{mwe}, \code{advmod}. For compound subjects and objects, they are \code{compound}, \code{nummod}, \code{det}, \code{advmod}, \code{amod}.
%     \item Finally, facets of a verb are identified through the following complements to the given verb: adverb modifier, prepositional and clausal complement.
% \end{itemize}
% %
% %\GW{this entire subsection assumes that the reader is fairly familiar with the NLP concepts, e.g., clausal complement, conjucts, possessives etc. -- I don't think we can make this assumption for WWW reviewers!}\\
% %\sr{I added a bit more of introduction to set the stage - concerning the core content not sure how to act on it, perhaps more examples also for what is not new? or alternatively we could go more abstractely?}
% We extend StuffIE's algorithm in the following ways: 
% \begin{enumerate}
%     \item The original algorithm includes all conjuncts of head words into one assertion, thus producing often overly specific assertions. In our method we break conjunctive objects (Table~\ref{tab:openie-examples}, row 1) and facets (Table~\ref{tab:openie-examples}, row 2) into separate assertions. Note that conjuncts should be connected by either \textit{``and''} or \textit{``or''}.
%     \item The original algorithm frequently returns assertions with empty objects. To only return complete triples, in such cases, we identify the nearest prepositional facet after its predicate and convert the facet into the assertion's object (Table~\ref{tab:openie-examples}, row 3).
%     \item We post-process special cases of sentences used for giving examples with the words: \textit{``like''}, \textit{``such as''} and \textit{``including''} to get finer-grained output (Table~\ref{tab:openie-examples}, row 4).
%     \item We convert all adverb modifiers of objects (besides those of predicates as in StuffIE) into facets. There are two types of modifiers we consider:
%     \begin{enumerate*}[label=(\roman*)]
%         \item direct adverb modifiers connected to object's head word through the edge \code{advmod} (Table~\ref{tab:openie-examples}, row 5);
%         \item the adverb in a noun phrase that follows the pattern ``adverb + adjective + object'' (Table~\ref{tab:openie-examples}, row 6).
%     \end{enumerate*}
% %    \item If the head of a subject (or an object) is a noun or a proper noun and its dependency parse is one of the following: \code{nsubj},  \code{dobj},  \code{nsubjpass},  \code{pcomp},  \code{pobj},  \code{dative},  \code{appos},  \code{attr} or  \code{ROOT}, the text spanning from the head's leftmost immediate child to itself will be extracted as the complete subject/object. Else, StuffIE's original algorithm will be used to find the compound subject/object. \sr{What is the issue here? Something that StuffIE missed (recall)? Or about precision? Perhaps example too?} \ph{Honestly I just didn't want to implement StuffIE's idea here, and just adapted the SpaCy noun\_chunk functionality as it has the same purpose as what StuffIE does. Perhaps we could drop this because I don't notice any major difference.}
% %    \item Facets linked to other assertions (i.e., nested facets) and negative assertions are discarded as those will not appear in our CSKB.
% \end{enumerate}
% %
% %\GW{much of this reads a bit like a long list of rules, heuristics, tricks etc. -- it leaves a bit of ad-hoc flavor! can we make this look more principled? for example, cast everything into rules with precondition and rewriting output?}
% %
% %\sr{Again not sure how to act here - we could change the style from StuffIE+diff into one long list of rules? But still, it really is a list of rules/heuristics.}
% Table~\ref{tab:openie-examples} gives a qualitative comparison of StuffIE's and our extraction results, while in the experiment section (Table~\ref{tab:openie}) we investigate their quantitative differences.

% \paragraph{Subject and predicate postprocessing} After OpenIE, we perform coreference resolution\footnote{\href{https://huggingface.co/coref}{https://huggingface.co/coref}} on paragraph level to resolve nominative pronouns occuring as subjects. For instance, the primarily extracted assertion \triple{they, have, long trunks} will be replaced by \triple{the elephants, have, long trunks} if ``they'' is resolved to ``the elephants''. This step helps improve the number of assertions extracted for each concept.
% % \GW{can we give an example, to get a feel for how difficult and how beneficial the co-ref resolution is here?}
% % \sr{Say what is resolved (nominative pronouns?) What is the approximate gain in terms of statements? 10\%? 50\%?}
% % \ph{I added an examples.}
% Then, all subjects are normalized by removing determiners and punctuation, and by lemmatizing head nouns.  Moreover, predicates are normalized so that main verbs are transformed to their infinite forms (e.g., ``has been found in'' $\rightarrow$ ``be found in'', ``is performing'' $\rightarrow$ ``perform''). Finally all extracted facet words are removed from predicates and objects.

% \paragraph{Facet type labeling} The extraction algorithm so far extracts facet values, but is unaware of their semantic type (e.g., ``spatial'' or ``causal''). For assigning semantic types, we fine-tune a RoBERTa~\cite{liu2019roberta} model to classify each facet into one of the aforementioned eight types. The input sequences of RoBERTa take the form: ``[CLS] subject [PRED] predicate [OBJ] object [FCT] facet [SEP]'', where [PRED], [OBJ] and [FCT] are special tokens used for marking the borders between different elements. The output vector of the [CLS] token is then passed to a fully-connected layer stacked with a soft-max layer on top of the transformer architecture to label the facet. Details on classifier training are in Section~\ref{sec:per-module-eval}.
% %\GW{what is the training data for the fine-tuning step? pos samples? neg samples??? whatis the loss function?}
% % SR: I put a forward reference

% \paragraph{Extraction of subgroups} Subgroups could be sub-species in case of animals, or refer to the target concept in different states, such as ``hunting cheetah'' and ``retired policeman''. For subject $s_0$, we collect all noun chunks (normalized as for triple subjects described above) ending with $s_0$ or any of its WordNet lemmas as potential candidates. %Note that chunks containing comparative adjectives (e.g., ``the biggest elephant'' and ``the younger cats'') are ignored.
% Semantically similar chunks, such as ``Canadian lynx'' and ``Canada lynx'', are then grouped using hierarchical agglomerative clustering (HAC) on average word2vec representations.% with distances measured by the cosine of the vector representations of the chunks computed by averaging element word vectors (using pre-trained word2vec~\cite{mikolov2013distributed}). 
% In addition, we leverage WordNet to distinguish antonyms, with which vector space embeddings typically struggle. Note that the subgroups are restricted to be less-than-5-words, and subgroups that syntactically contain other subgroups are disregarded (e.g., ``old male Canadian lynx'' is grouped with ``Canadian lynx''). In addition, a chunk will be ignored if it is a named entity (e.g., ``Will Smith'' for the concept ``smith''). Finally we use WordNet hyponyms to remove spurious subgroups, e.g., ``sea lion'' and ``ant lion'' w.r.t.\ ``lion''.

% \paragraph{Extraction of related aspects} Given subject $s_0$ and its WordNet lemmas $L_{s_0}$, related aspects of the subject are extracted from noun chunks collected from two sources:
% \begin{enumerate}[label=(\roman*)]
%     \item \textit{Possessive noun chunks} where the possessives refer to any lemma in $L_{s_0}$, for example, ``elephant's diet'' and ``their diet'' (with resolution to ``elephant'');
%     \item \triple{$s$, $p$, noun chunk} triples where $s \in L_{s_0}$ and $p$ is one of the following verb phrases: ``have'', ``contain'', ``be assembled of'' or ``be composed of''.
% %\GW{this is a good example for my earlier comments: what are possessive noun chunks (even I would have to guess)? is this a principle rule here, or just an ad-hoc trick?} \sr{I suppose this step has higher yield than the first? If so I would invert the order and say so. Examples of possessive noun chunks would be ``elephant's diet'', ``their diet'' (with resolution to ``elephant'', ``the diet of elephants''? Please confirm which cases we cover then I'll rewrite this.} \ph{We only cover ``elephant's diet'' and ``their diet'' (with resolution to ``elephant''), the case of ``the diet of elephants'' is not processed. I don't have comprehensive statistics but a quick look at ``lion'' data says that the 2nd case has higher yield.}
% \end{enumerate}
% In order to prevent too specific aspects (e.g., ``large paws'' or ``short tails''), only compound nouns (if applicable) or nouns in these \textit{noun chunks} are then extracted as aspects of $s_0$. For example, if we observe \triple{lynx, have, black ear tuft}, then the adjective ``black'' is ignored and ``ear tuft'' will be extracted instead of only extracting the head noun ``tuft''.

% \paragraph{Retained assertions}
% For each primary subject, a separate set of documents is processed, and the output of this stage are three sets of assertions: Assertions for the primary subject $s_0$, assertions for its subgroups, and assertions for its aspects. These are selected as follows.

% %\GW{is this a filtering/selection step, or some of re-grouping/bundling several assertions? what is the intuitive goal here? and the quantitative objective?}\\

% As assertions for the main subject and its subgroups we simply retain all assertions that have a subject that matches a WordNet lemma of the primary subject, or the name of one of its subgroups.

% %Similarly, for the subgroup assertions, any statement is retained whose subject matches an identified subgroup, i.e., a noun chunking ending in the main subject.

% The case of aspect assertions is slightly more complex, we merge three cases:
% \begin{enumerate}
%     \item Assertions that have a subject which is among the previously identified aspects;
%     \item Assertions that have a subject among the lemmas of the main subject, and an object which is a noun chunk consisting of an aspect $t \in asp_{s_0}$ as the head noun and an adjectival modifier $adj$ of $t$. For instance, from the assertion \triple{elephant, have, a long very trunk} we infer that \triple{elephant trunk, be, long, DEGREE: very}.
%     %\sr{Give example - what does this case catch??} \ph{One example could be <elephant; have; a very long trunk> then <elephant trunk; be; long; degree: very>}
%     \item All noun chunks that follow the pattern \emph{``possessive + adj + t''} (e.g., ``elephant's long trunks''), where $possessive$ refers to any lemma in $L_{s_0}$, \textit{adj} is an adjectival modifier of $t$, and $t \in asp_{s_0}$.
% \end{enumerate}
% Results from the latter two cases are transformed into \triple{t, be, adj, F} assertions where the facets $F$ are extracted from adverb modifiers of \textit{adj}.
% %Finally, we have $S_1 \cup S_2$ as the final set of aspect assertions.
% %\sr{I tried to rewrite this, but I don't understand the second case - please explain by example, and also recheck what I wrote for case 3.} \ph{Case 3 looks good!}


% %Given a subject $s_0$ and its WordNet lemmas $L_{s_0}$, its subgroup set $sg_{s_0}$, aspect set $asp_{s_0}$ and the assertion set $A$ returned by our OpenIE module, we proceed to select commonsense assertions of $s_0$ which include set of general assertions $GA_{s_0}$, set of subgroup assertions $SGA_{s_0}$ and set of aspect assertions $ASPA_{s_0}$.
% %\begin{enumerate}
% %    \item $GA_{s_0} = \{a \mid a \in A, \textit{subject}(a) \in L_{s_0}\}$
% %    \item $SGA_{s_0} = \{a \mid a \in A, \textit{subject}(a) \in sg_{s_0}\}$
% %    \item We construct $S_1 = \{a \mid a \in A, \textit{subject}(a) \in asp_{s_0}\}$. Then we collect more assertions from the following two sources.
% %    \begin{enumerate}[label=(\roman*)]
% %        \item The first source is \triple{$s, p, o$} triples where $s \in L_{s_0}$, and $o$ is a noun chunk which consists of an aspect $t \in asp_{s_0}$ as the head noun and an adjectival modifier $adj$ of $t$.
% %        \item The other source includes all noun chunks following the pattern \emph{``possessive + adj + t''}, whereas $possessive$ refers to any lemma in $L_{s_0}$, \textit{adj} is an adjectival modifier of $t$, and $t \in asp_{s_0}$.
% %    \end{enumerate}
% %    Candidates from these two sources are then transformed into a second sub-set $S_2 = \{(t, \textit{be}, adj, F)\}$ whereas the facets are extracted from adverb modifiers of $adj$. Finally, we have $ASPA_{s_0} = S_1 \cup S_2$ as the final set of aspect assertions.
% %\end{enumerate}




% \subsection{Knowledge Consolidation}
% %
% Natural language is rich in paraphrases, and consequently, the extraction pipeline so far produces frequently assertions that carry the same or nearly the same meaning. Identifying and clustering such assertions is necessary, in order to avoid redundancies, and get better frequency signals for individual assertions.

% \paragraph{Triple clustering} Because extraction is done for each concept separately, we only need to cluster predicate-object pairs. First, we train a RoBERTa model to detect if two given triples are semantically similar (for setup details see Sec.~\ref{sec:per-module-eval}). Confidence scores given by the model are then used to compute distances for the HAC algorithm to group assertions into clusters. Given two assertions \triple{$s, p_1, o_1$} and \triple{$s, p_2, o_2$}, the input sentence given to RoBERTa is: ``[CLS] [SUBJ] $p_1$ [U-SEP] $o_1$ [SEP] [SUBJ] $p_2$ [U-SEP] $o_2$ [SEP]'', where [SUBJ] and [U-SEP] are new special tokens introduced to replace identical subjects and mark the borders between predicates and objects, respectively. The output vector of the [CLS] token is used for the classification purpose in the same way as in the model used for facet labeling described above.

% Ideally one would compute the full distance matrix between all assertions (an $n\times n$ matrix for $n$ triples), but given that pretrained language models (LM) are exceedingly resource-intensive, this quadratic computation would be expensive even for moderate assertion sets. We therefore reduce the computational effort by pre-filtering the set of pairs to be compared by the pretrained LM.
% \begin{enumerate}
%     \item The assertions are sorted in decreasing order of frequency.
%     \item We compute cosine similarities between vector representations of predicate-object pairs, using word2vec embeddings. This can be done very fast with parallel matrix multiplication.
%     \item For each assertion $a_i$, we then only compute the RoBERTa-based distances with the top-$k$ most similar assertions (ranked by word2vec-based similarities) that succeed $a_i$ in the sorted list (the sorted list helps us focus on salient assertions). All other pairs get the distance of $1.0$. This produces a ``sparse'' distance matrix for $n$ assertions.
%     \item For clustering, we use the HAC algorithm with single linkage, because it only looks at the most similar pairs between two clusters. That helps to reduce the chance of missing similar triples whose similarities were not computed by RoBERTa in the third step.
% \end{enumerate}
% After clustering, the most frequent assertion inside each cluster is used as representative.

% \paragraph{Facet value clustering}
% Facet values may similarly exhibit redundancy, for example, the degree facet may come with values ``often'', ``frequently'', ``mostly'', ``regularly'', etc. Also, sources may occasionally mention odd values. We combat both by clustering facet values per facet type, and retaining only the one with strongest support.
% %\GW{what is the goal here? merge and unify equivalent facets per assertion? or group complementary ones together; i.e., a form of union or re-assignment?}\\
% %\sr{added explanation above}

% Considering the small number of facet values per assertion and facet type (usually less than 5), we utilize simple methods for clustering. Specifically, given the list of values, we use the HAC algorithm to cluster values which are adverbs, in which distance between two values is measured by the cosine distance of their word2vec presentations. Other values are grouped if they have the same head word (e.g., ``during evening'' and ``in the evening'' go to one same cluster). Similarly, the most frequent value inside a cluster is used as representative of that cluster. %If multiple values remain after clustering, we only retain the cluster with the highest frequency. 
% % \ph{As noted before, we in fact allow multiple values per facet type.}
% % \sr{Great, I must have missed that!}

%\ph{From here, all is new material}
%\oldmaterial

==> tables_backup/tables.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lrrrrrrrrrrr}
\toprule
\multirow{4}{*}{\textbf{CSK resource}} & \multicolumn{4}{c}{\textbf{Precision (\%)}} & \multicolumn{6}{c}{\textbf{Recall (\%)}} & \textbf{Size}\\
\cmidrule(l){2-5} \cmidrule(l){6-11} \cmidrule(l){12-12}
& \multicolumn{2}{c}{\textbf{Saliency@10}} & \multicolumn{2}{c}{\textbf{Typicality (all)}} & \multicolumn{3}{c}{\textbf{Top-100 assertions/subject}} & \multicolumn{3}{c}{\textbf{All assertions}} &  \\
% \midrule
\cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-8} \cmidrule(l){9-11} \cmidrule(l){12-12}
& \textbf{Salient} & \textbf{Unsalient} & \textbf{Typical} & \textbf{Untypical} & \textbf{t = 0.96} & \textbf{t = 0.98} & \textbf{t = 1.00} & \textbf{t = 0.96} & \textbf{t = 0.98} & \textbf{t = 1.00} & \textbf{\#spo} \\
\bigtableline
\multicolumn{3}{l}{\textit{Crowdsourced}} & & & & & & & & &  \\
\bigtableline
ConceptNet~\cite{conceptnet} & 79.2 & 20.4 & 96.0 & 3.6 & 5.29 & 3.39 & 1.10 & 5.47 & 3.53 & 1.13 & 0.5M \\
\bigtableline
\multicolumn{3}{l}{\textit{Generative}} & & & & & & & & &  \\
\bigtableline
COMET~\cite{comet-atomic-2020} & 55.2 & 43.6 & 78.9 & 20.1 & - & - & - & - & - & - & - \\
\bigtableline
\multicolumn{3}{l}{\textit{Extractive}} & & & & & & & & & \\
\bigtableline
TransOMCS~\cite{DBLP:conf/ijcai/ZhangKSR20} & 40.4 & 59.0 & 51.4 & 46.2 & 4.04 & 3.24 & 1.85 & 19.70 & 16.47 & 9.06 & 18.5M \\
\bigtableline
TupleKB~\cite{mishra2017domain} & 36.0 & 63.0 & \textbf{92.0} & \textbf{6.4} & 3.57 & 1.99 & 0.41 & 4.32 & 2.49 & 0.58 & 0.3M \\
\bigtableline
Quasimodo~\cite{quasimodo} & 38.8 & 60.2 & 67.8 & 31.0 & 11.05 & 9.47 & 5.17 & \textbf{21.87} & \textbf{19.36} & \textbf{10.88} & 6.3M \\
\bigtableline
\ascent{}~\cite{ascent} & 60.0 & 38.6 & 79.2 & 15.8 & 9.60 & 7.02 & 3.17 & 17.09 & 12.62 & 5.82 & 8.6M \\
\bigtableline
\ascentpp{} & \textbf{68.8} & \textbf{30.8} & 88.4 & 8.8 & \textbf{12.70} & \textbf{10.70} & \textbf{5.90} & 17.54 & 14.64 & 7.95 & 2.0M \\
\bottomrule
\end{tabular}
\caption{Intrinsic evaluation results of different CSK resources.
% \sr{To be merged with recall tables and size into one main result table}
% \ph{TODO: tune the vertical line.}
}
\label{tab:eval-triple-quality}
\end{table*}

\begin{table}[t]
    \centering
    \begin{tabular}{lrrrr}
    \toprule
    \multirow{2}{*}{\textbf{CSKB}} & \multicolumn{2}{c}{\textbf{Typicality@10}} & \multicolumn{2}{c}{\textbf{Typicality (Random)}} \\
    \cmidrule(l){2-3} \cmidrule(l){4-5}
     & \textbf{Typical} & \textbf{Untypical} & \textbf{Typical} & \textbf{Untypical} \\
    \cmidrule(l){1-1} \cmidrule(l){2-3} \cmidrule(l){4-5}
    \ascent{}~\cite{ascent} & 87.6 & 6.0 & 74.4 & 11.2 \\
    \cmidrule(l){1-1} \cmidrule(l){2-3} \cmidrule(l){4-5}
    \ascentpp{} & \textbf{93.6} & \textbf{2.8} & \textbf{84.2} & \textbf{10.0} \\
    \bottomrule
    \end{tabular}
    \caption{Typicality evaluation of \ascent{} and \ascentpp{}.}
    \label{tab:ascent-vs-ascentpp}
\end{table}
